Reactive Human-to-Robot Handovers of Arbitrary Objects

Human-robot object handovers have been an actively studied area of robotics over the past decade; however, very few techniques and systems have addressed the challenge of handing over diverse objects with arbitrary appearance, size, shape, and rigidity. In this paper, we present a vision-based system that enables reactive human-to-robot handovers of unknown objects. Our approach combines closed-loop motion planning with real-time, temporally-consistent grasp generation to ensure reactivity and motion smoothness. Our system is robust to different object positions and orientations, and can grasp both rigid and non-rigid objects. We demonstrate the generalizability, usability, and robustness of our approach on a novel benchmark set of 26 diverse household objects, a user study with naive users (N=6) handing over a subset of 15 objects, and a systematic evaluation examining different ways of handing objects. More results and videos can be found at https://sites.google.com/nvidia.com/handovers-of-arbitrary-objects.

==> 9_redacted.tex <==

\begin{table*}[bt]
    \centering
    \begin{tabular}{l cc cc cc cc}
    \toprule
         & \multicolumn{2}{c}{Banana} & \multicolumn{2}{c}{Bottle} & \multicolumn{2}{c}{Cereal Box} & \multicolumn{2}{c}{Overall} \\
         Grasp Type & Time (s) & Success (\%) & Time (s) & Success (\%) & Time (s) & Success (\%) & Time (s) & Success (\%) \\
    \midrule
        Naive GraspNet & $9.64 \pm 0.73$ & 100\% & $10.77 \pm 1.58$ & 100\% & $8.76 \pm 1.02$ & 100\%
        & $9.73 \pm 1.43$ & 100\% \\ 
        Temporal-GraspNet & $11.53 \pm 2.84$ & 100\% & $19.43 \pm 5.68$ & 75\% & $10.58 \pm 2.00$ & 75\%
        & $14.41 \pm 5.79$ & 82\% \\
        Temporal-GraspNet++ & $11.87 \pm 0.33$ & 100\% & $8.46 \pm 0.30$ & 100\% & $10.42 \pm 1.50$ & 75\%
        & $10.27 \pm 1.65$ & 90\% \\
    \bottomrule
    \end{tabular}
    \caption{Baseline comparison for various objects. ``Naive'' resamples grasps on every iteration, and therefore will rely entirely on the cost function for grasp consistency. ``Temporal'' will attempt to grab the best initial grasp, and will try to choose the best grasp at each step. Reactive grasping with GraspNet only resulted in a high failure rate, as the robot would oscillate between goals too much.}
    \label{tab:baseline}
\end{table*}

\subsection{Ablation Study}

\begin{itemize}
    \item \textbf{Object Center}: in this variation, we use the object center computed from the object segmentation and a fixed grasp orientation to determine the target grasp.
    \item \textbf{Naive GraspNet}: given the segmented point cloud of the object, we use the GraspNet to generate a set of candidate grasps for each time step independently. 
    % Then we select the grasp with highest score to execute the handover. 
    \item \textbf{Temporal-GraspNet}: instead of sampling grasps for each time step, we use the temporal refinement in Sec.~\ref{} to generate grasps that are consistent over time, and attempt to take the closest grasp to the hand every time.
    \item \textbf{Temporal-GraspNet++ (Ours)}: instead of execute the grasp with the highest score, we select the grasp according to Sec.~\ref{} to maximize the smoothness and naturalness of the robot motion.
\end{itemize}
Describe how we do this experiment.

\textbf{Results. }
% can we compare the proposed system with IROS20 system on blocks (time/success rate/collision with hand)s?


